An Objective for Hierarchical Clustering in Euclidean Space and its Connection to Bisecting K-means

This paper explores hierarchical clustering in the case where pairs of points have dissimilarity scores (e.g. distances) as a part of the input. The recently introduced objective for points with dissimilarity scores results in every tree being a 1/2 approximation if the distances form a metric. This shows the objective does not make a significant distinction between a good and poor hierarchical clustering in metric spaces. Motivated by this, the paper develops a new global objective for hierarchical clustering in Euclidean space. The objective captures the criterion that has motivated the use of divisive clustering algorithms: that when a split happens, points in the same cluster should be more similar than points in different clusters. Moreover, this objective gives reasonable results on ground-truth inputs for hierarchical clustering. The paper builds a theoretical connection between this objective and the bisecting k-means algorithm. This paper proves that the optimal 2-means solution results in a constant approximation for the objective. This is the first paper to show the bisecting k-means algorithm optimizes a natural global objective over the entire tree.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> stash.tex <==

\begin{definition} \label{def:generate_ultrametric}
A weighted graph $G=(V,E,w)$ is a \emph{dissimilarity graph generated from an ultrametric}, if there exists an ultrametric $(X,d)$ such that $V \subseteq X$, and for every $x,y \in V$, $x \neq y$, $e = ( x , y )$ exists, and $w(e)=f(d(x,y))$, where $f:\mathbb{R}_+ \mapsto \mathbb{R}_+$ is a non-decreasing function.
\end{definition}

In our context where we use Euclidean distances as dissimilarity scores, we let the weight function $f(d(x,y))$ equal $d(x,y)$. Naturally, we convert the input point set $V$ into a complete graph $G = (V,E,w)$, where for every edge $e=(x,y)$, $w(e)=d(x,y)$. Next, following \citet{cohen2018hierarchical}, we define \emph{generating trees}, which are considered the most well-behaving \hc trees for a ground-truth input.
\begin{definition} \label{def:generating_tree}
If a graph $G=(V,E,w)$ is generated by ultrametric, a binary tree $T$ is a generating tree for $G$ if it satisfies the following properties:
\begin{enumerate}
\item It has $|V|$ leaves and $|V| - 1$ internal nodes. Let $L$ denote its leaves and $L$ corresponds to the points in $V$. 
\item There exists a weight function $W: \mathcal{N} \mapsto \mathbb{R}_+$. For $N_1,N_2 \in \mathcal{N}$, if $N_1$ is on the path from $N_2$ to the root, $W(N_1) \geq W(N_2)$. For every $x,y \in V$, $w( (x,y) ) = W(LCA_T(x,y))$, where $LCA_T(x,y)$ denotes the Least Common Ancestor of leaves corresponding to $x$ and $y$ in $T$.
\end{enumerate}
\end{definition}


We give an alternative description of a generating tree, which provides intuition for why it is considered the best tree on such inputs. The value $W(LCA_T(x, y))$ can be interpreted as the weight (distances) of edges cut in split at the LCA of $x$ and $y$. Naturally, the higher up this LCA is, the larger the distance should be. For each ground-truth input graph, there is always a generating tree $T$, which separates the longest edges in every split.

\citet{cohen2018hierarchical} proposed that for a ground-truth input graph as defined in Definition~\ref{def:generate_ultrametric}, if there exists any corresponding generating tree $T$, it is considered one of the best solutions among all the solutions, and thus should be one of the optimal solutions for the \hc objective function used.

\subsection{Optimality of Generating Trees}
Now we prove that for every tree $T$  that is a generating tree for the graph $G=(V,E,w)$ generated from ultrametric in Euclidean space, it gets full revenue for \probname function introduced in this paper. 



\begin{lemma} \label{lem:generating_tree_cuts_biggest_distances}
A binary tree $T$, with $|V|$ leaves corresponding to the points in $V$ and $|V|-1$ internal nodes, is a generating tree for $G$ if and only if it satisfies the following property:
\begin{itemize}
    \item For every split $A \cup B \rightarrow (A,B)$ from top to bottom, $\forall{i \in A, j \in B}, d(i,j) = \max_{x \in A, y \in B }d(x,y)$.
\end{itemize}
\end{lemma}

Every ground-truth input has at least one generating tree, as stated in the following theorem.

\begin{theorem} \label{thm:always_generating_tree}
For every graph $G=(V,E,w)$ generated from some ultrametric, there is always a generating tree $T$ as defined in Definition~\ref{def:generating_tree}.
\end{theorem}

Using Lemma~\ref{lem:generating_tree_cuts_biggest_distances}, the optimality of $T$ is proved by arguing every split gives a revenue of $1$ for every pair of points it separates.

\begin{theorem} \label{thm:generating_tree_optimal}
A generating tree $T$ for some graph $G = (V,E,w)$ generated from ultrametric is optimal for \probname function. 
\end{theorem}

